Agile Interception of a Flying Target using Competitive Reinforcement Learning

This article presents a solution to intercept an agile drone by another agile drone carrying a catching net. We formulate the interception as a Competitive Reinforcement Learning problem, where the interceptor and the target drone are controlled by separate policies trained with Proximal Policy Optimization (PPO). We introduce a high-fidelity simulation environment that integrates a realistic quadrotor dynamics model and a low-level control architecture implemented in JAX, which allows for fast parallelized execution on GPUs. We train the agents using low-level control, collective thrust and body rates, to achieve agile flights both for the interceptor and the target. We compare the performance of the trained policies in terms of catch rate, time to catch, and crash rate, against common heuristic baselines and show that our solution outperforms these baselines for interception of agile targets. Finally, we demonstrate the performance of the trained policies in a scaled real-world scenario using agile drones inside an indoor flight arena.

==> background.tex <==
%=============================================================================================================================
\section{Background}

\subsection{Reinforcement Learning}

Reinforcement Learning is a type of machine learning for sequential decision-making.
In a \textit{rollout} phase, an \textit{agent} interacts with an uncertain \textit{environment} which provides it with a \textit{partial observations} of its \textit{state}, takes a series of \textit{actions} following a \textit{policy} and receives a scalar feedback in the form of \textit{rewards}.
These sequences of observe-act-reward, repeated over time, form the \textit{rollouts}.
The collected rollouts are then used to update the policy in a learning phase, which will then be employed in the rollout phase of the next training iteration.
\textcolor{red}{\em This subsection should be a brief presentation of MARL, with a focus on the challenges it raises and an introduction to the CTDE framework and the most popular algorithms.}


\subsection{Competitive self-play}
\textcolor{red}{\em This subsection lists a few methods used to train agents on competitive or mixed-competitive problems. Such as population-based methods : self-play, fictitious self-play (eg AlphaGo, AlphaStar),  asymmetric self-play (eg. ), PSRO; regret minimization methods; .
And then explain the principle of asymmetric self-play, and why it is used in our work. We briefly explain the limitation of classical SP and how Fictitious Self Play can solve it. Self-play has convergence garantee for symmetrical zero-sum games, which our case is not part of. Later in the document, we will explain how our game is a "near-zero-sum" game which will allows us to use Fictitious Self Play.}

SP is a training methods where an agent plays against oneself without any direct supervision. 
It yields excellent performance in challenging tasks such as Go, Poker,
Simulated Sumo, Dota 2, StarCraft II, and more. 
However, it famously suffers from the problem of overfitting to a single opponent and forgetting how to win against past versions.
Fictitious Self-Play is one solution to solve this problem. Each agent learns a best response to the empirical frequency distribution of the opponent’s past strategies. In practice, each agent periodically freezes its policy while the other agent adapt to that frozen policy. Then the roles swap. 
Fictitious play, each agent learns a best response to the empirical frequency distribution of the opponent’s past strategies. Each agent periodically freezes its policy while the other agent adapt to that frozen policy. Then the roles swap. 
Currently, there are three primary competitive SP methods : SP Latest, and SP Best, where each agent compete against the last or the best version of the other agent, and SP with a random past agent.

